Traditional and Heavy-Tailed Self Regularization in Neural Network Models

Random Matrix Theory (RMT) is applied to analyze the weight matrices of Deep Neural Networks (DNNs), including both production quality, pre-trained models such as AlexNet and Inception, and smaller models trained from scratch, such as LeNet5 and a miniature-AlexNet. Empirical and theoretical results clearly indicate that the empirical spectral density (ESD) of DNN layer matrices displays signatures of traditionally-regularized statistical models, even in the absence of exogenously specifying traditional forms of regularization, such as Dropout or Weight Norm constraints. Building on recent results in RMT, most notably its extension to Universality classes of Heavy-Tailed matrices, we develop a theory to identify \emph{5+1 Phases of Training}, corresponding to increasing amounts of \emph{Implicit Self-Regularization}. For smaller and/or older DNNs, this Implicit Self-Regularization is like traditional Tikhonov regularization, in that there is a `size scale' separating signal from noise. For state-of-the-art DNNs, however, we identify a novel form of \emph{Heavy-Tailed Self-Regularization}, similar to the self-organization seen in the statistical physics of disordered systems. This implicit Self-Regularization can depend strongly on the many knobs of the training process. By exploiting the generalization gap phenomena, we demonstrate that we can cause a small model to exhibit all 5+1 phases of training simply by changing the batch size.

==> gen_gap_paper6shortTR_empirical_explicitReg.tex <==

\subsection{Effect of explicit regularization}
\label{sxn:main-explicit}




\paragraph{Transition in Layer Entropy and Stable Rank.}

In each case (of adding $L_2$ norm weight regularization or Dropout to the baseline results), we observe a greater decrease in the complexity metrics (Entropies and Stable Ranks) with explicit regularization than without, consistent with expectations; and we see that explicit regularization affects these metrics dramatically.
Here too, the Layer Entropy decreases relatively more for FC2, and the Stable Rank decreases relatively more for FC1.  %% indicating non-uniformity across layers for both explicit regularization and implicit Self-Regularization.





\paragraph{Eigenvalue Spectrum: Comparisons with RMT.}


When explicit Dropout regularization is added, the eigenvalues in the spike are pulled to much larger values (consistent with a much more implicitly-regularized model).
A subtle but important consequence of this regularization%
\footnote{This is seen in Figure~\ref{fig:esd-alexnet-fc1-10runs} in the baseline, but it is seen more clearly here, especially for FC2 in Figure~\ref{fig:mini-alexnet-dropout-esd-good-fits}.}
is the following: this leads to a smaller bulk MP variance parameter $\sigma_{mp}^2$, and thus smaller values for $\lambda^{+}$, when there is a more prominent spike.
Similar results for the ESD for layers FC1 and FC2 of MiniAlexNet are seen with explicit $L_2$ norm weight regularization. 







\paragraph{Eigenvalue localization.}

We observe that eigenvector localization tends to be more prominent when the explicit regularization is stronger, presumably since explicit ($L_2$ Weight Norm or Dropout) regularization can make spikes more well-separated from the bulk. 



